Exploring the Landscape of Distributed Graph Sketching

Recent work has initiated the study of dense graph processing using graph sketching methods, which drastically reduce space costs by lossily compressing information about the input graph. In this paper, we explore the strange and surprising performance landscape of sketching algorithms. We highlight both their surprising advantages for processing dense graphs that were previously prohibitively expensive to study, as well as the current limitations of the technique. Most notably, we show how sketching can avoid bottlenecks that limit conventional graph processing methods. Single-machine streaming graph processing systems are typically bottlenecked by CPU performance, and distributed graph processing systems are typically bottlenecked by network latency. We present Landscape, a distributed graph-stream processing system that uses linear sketching to distribute the CPU work of computing graph properties to distributed workers with no need for worker-to-worker communication. As a result, it overcomes the CPU and network bottlenecks that limit other systems. In fact, for the connected components problem, Landscape achieves a stream ingestion rate one-fourth that of maximum sustained RAM bandwidth, and is four times faster than random access RAM bandwidth. Additionally, we prove that for any sequence of graph updates and queries Landscape consumes at most a constant factor more network bandwidth than is required to receive the input stream. We show that this system can ingest up to 332 million stream updates per second on a graph with $2^{17}$ vertices. We show that it scales well with more distributed compute power: given a cluster of 40 distributed worker machines, it can ingest updates 35 times as fast as with 1 distributed worker machine. Landscape uses heuristics to reduce its query latency by up to four orders of magnitude over the prior state of the art.

==> acknowledgements.tex <==
\balance
\subsection*{Acknowledgments}
We thank the authors of \graphzep for providing source code, datasets, and graph stream generators.

==> appendices/network_experiment_full.tex <==
\section{Network Communication}
\label{app:networkcomm}
\input{figures/network}
Throughout our scaling experiments in Section ~\ref{subsec:scaling} we observe a constant amount of network communication used; approximately $1.6$ times the size of the input stream. Moreover, we demonstrate experimentally that this bandwidth use is near-optimal: Figure~\ref{fig:network} and~\ref{fig:network_throughput} validate our claims that \sysname's vertex-based batches are large enough to amortize the communication costs over the CPU cost of processing sketch updates. Figure~\ref{fig:network_throughput} shows that OpenMPI messages containing vertex-based batches hit the half-bandwidth point when they contain at least several thousand updates. Figure~\ref{fig:network_latency} shows that at this batch size the costs of serializing and sending the message are quite small: the latency is less than $0.1$ millisecond. We configure \sysname to produce vertex-based batches a factor $1.2 \times$ larger than a sketch delta. For a graph on $2^{17}$ vertices, the size of a vertex-based batch is $42$KiB or $10,670$ edge updates. We conclude that \sysname successfully amortizes away the network communication costs, enabling its impressive scaling.

==> appendices/pht_design.tex <==

\section{\Treename Design Considerations}
\label{app:pipeline_design}
To avoid the performance detriments of cascading flushes, in which a flush triggers another flush of one of its children, we implement optimizations inspired by the work in~\cite{BenderDaFa20Flushing}. Cascading flushes (and flushes to leaves in general) are particularly expensive for this problem; The latency difference between accessing the root nodes (which are likely stored in L1 or L2) and the leaf nodes (which are likely stored in RAM) is approximately a factor of 20-80\cite{Brett16}. Specifically, at each subsequent thread-local level of the DAG the buffer size and fan-out are both doubled. This double-doubling means that, in expectation, when we flush a root node, we flush $\frac{1}{4}$ level two nodes, $\frac{1}{16}$ level three nodes, etc. It also helps these buffers fit into the different levels of cache; our tree grows approximately as fast as cache does. This dramatically improves the latency of each \treename root flush as we no longer flush an entire root-to-leaf path in expectation. Our implementation uses $5$ total levels, $3$ of which are thread-local. The $5$th level are called leaf buffers and are treated as a special case; there are $V$ buffers, each of size $O(\alpha\log^2\nodesize)$.

==> appendices/prior_connectivity.tex <==
\section{Prior Work in Connectivity Sketching}
\label{app:alg}

We summarize \algname and \graphzep, respectively Ahn \etal's~\cite{Ahn2012} and Tench \etal's~\cite{graphzeppelin} semi-streaming algorithms for computing a spanning forest (and therefore the connected components) of a graph.  These algorithms have some overlap so for conciseness we describe them in parallel and note where they differ.

For each vertex $v_i$ in $G$, define the \defn{characteristic vector} $\charvec_i$ of $v_i$ to be an $\binom{n}{2}$-dimensional vector indexed by the set of possible edges in $\graph$.  $\charvec_i[(j,k)]$ is only nonzero when $i = j$ or $i = k$ and edge $(j,k) \in \edges$.  That is, $\charvec_i \in \{-1,0,1\}^{\binom{\nodesize}{2}}$ s.t. for all $0 \leq j < k < {\binom{\nodesize}{2}}$: 
$$\charvec_i[(j,k)] = \left\{ \begin{array}{ll}
            1 & \quad i = j \text{ and }(v_j, v_k) \in \edges \\
            -1 & \quad i = k \text{ and }(v_j, v_k) \in \edges \\
            0 & \quad \text{otherwise} 
            
        \end{array}\right\}%\{1$ $if$ $i = j$ $and$ $(v_j, v_k) \in E, -1$ $if$ $i = k$ $and$ $(v_j, v_k) \in E, 0 \text{ otherwise}\}
$$

%The characteristic vector $a_i$ is a 1-dimensional vector indexed by the set of possible edges in $\graph$.  $a_i[(j,k)]$ is only nonzero when $i = j$ or $i = k$ and edge $(j,k) \in \edges$.

These characteristic vectors have an important property that is vital for computing connectivity: For any $S \subset \nodes$, the sum of the characteristic vectors of the vertices in $S$ is a direct encoding of the edges across the cut $(S, \nodes \setminus S$).  That is, let $x = \sum_{v \in S} \charvec_v$ and then % $x\in \{-1,0,1\}^{\binom{n}{2}}$ and 
$|x[(j,k)]| = 1$ iff $(j,k) \in E(S, \nodes \setminus S)$.

%\input{figures/supernode_example}

It is simple to update the characteristic vectors as stream updates arrive. Initialize $\charvec_i = \{0\}^{\binom{\nodesize}{2}}$ for all $i$. For each stream update $s = ((u,v), \Delta)$, set $\charvec_u[u,v] += \Delta$ and $\charvec_v[u,v] += -\Delta$.Using these vectors, we immediately have a (very inefficient) algorithm for computing the connected components from a stream by running Boruvka's algorithm~\cite{boruvka} for finding a spanning forest as follows.  For the first round of the algorithm, from each $a_i$ arbitrarily choose one nonzero entry $(w,y)$ (an edge in $\edges$ s.t. w = i or y = i).  Add $e_i$ to the spanning forest.  For each connected component $C$ in the spanning forest, compute the characteristic vector of $C$: $\charvec_C = \sum_{v\in C} \charvec_v$.  Proceed similarly for the remaining rounds of Boruvka's algorithm: in each round, choose one nonzero entry from the characteristic vector of each connected component and add the corresponding edges to the spanning forest.  Sum the characteristic vectors of the component vertices of the connected components in the spanning forest. Repeat until no new merges are possible.  This takes at most $\log(\nodesize)$ rounds.

The key idea to make this a small-space algorithm is to use $\ell_0$-sampling ~\cite{l0sketch} to run this version of Boruvka's algorithm by compressing each characteristic vector $\charvec_i$ into a data structure of size $O(\log^2(\nodesize))$ that can return a nonzero entry of $\charvec_i$ with high probability.  For all $\ell_0$ samplers discussed in this paper, $\sketch(\charvec)$ is a vector and adding two sketches is equivalent to adding their vectors elementwise. The $\ell_0$ sampler may fail to sample an element; for Boruvka's algorithm to succeed in $O(\log\nodesize)$ rounds, each sampler must fail with at most constant probability.

\algname uses an $\ell_0$ sampler of Cormode \etal:

\begin{theorem} (Adapted from ~\cite{l0sketch}, Theorem 1):
Given a 2-wise independent hash family $\mathcal{F}$ and an input vector $x \in \mathbb{Z}^n$, there is an $\ell_0$-sampler using $O(\log^2(n)\log(1/\delta))$ space that succeeds with probability at least $1 - \delta$.
\end{theorem}

\graphzep uses \cubesketch, an $\ell_0$ sampler that is purpose-built for sketching characteristic vectors and as a result reduces average-case update cost:

\cubesketchthm*

%\david{clarify support finding only?}
\sysname uses a new, improved $\ell_0$ sampler which we call \sketchname which improves worst-case update time to $O(\log(n))$ and reduces space by a constant factor. It supports the same operations as \cubesketch and is used to run Boruvka in the same way. We summarize \cubesketch and present \sketchname in Section~\ref{subsec:cameo}. 
%we choose to use \cubesketch for $\ell_0$ sampling because it performs better in practice~\cite{graphzeppelin}.\david{now we say we use our own thing which is better than cubesketch}

We denote the $\ell_0$ sketch of a vector $x$ as $\sketch(x)$.  Since the sketch is linear, $\sketch(x) + \sketch(y) = \sketch(x+y)$ for any vectors $x$ and $y$.  This allows us to process stream updates as follows: we maintain a running sum of the sketches of each stream update, which is equivalent to a sketch of the vector defined by the stream. That is, let $\charvec_i^t$ denote $\charvec_i$ after stream prefix $\stream_t$. For the $j$th stream update $\streamelement_j = ((i,x),\Delta)$ we obtain $\sketch(\charvec_i^j) = \sketch(\streamelement_j) + \sketch(\charvec_i^{j-1})$. For each stream update $\streamelement_j$, \algname computes $\sketch(\charvec_i^j)$ as soon as $\streamelement_j$ arrives from the input stream. In contrast, \graphzep inserts $\streamelement_j$ into a \defn{gutter tree} of size $O(\nodesize \log^3(\nodesize))$ that write-efficiently collects updates by endpoint. When $O(\log^3(\nodesize))$ updates have been collected for vertex $i$, $\streamelement_j$ and all other collected updates for vertex $i$ are added to $\sketch(\charvec_i)$. The gutter tree allows stream ingestion to be done I/O optimally when the gutter tree and sketches are stored on disk; we omit the details here.
mark
Linearity also allows Ahn \etal to emulate the merging step of Boruvka's algorithm by summing the sketches of all vertices in each connected component.  They require $\log\nodesize)$ independent $\ell_0$ sketches for each $v \in \nodes$, one for each round\footnote{Ahn \etal~\cite{Ahn2012} the authors note that adaptivity concerns require the use of new sketches for each round of Boruvka's algorithm.}, so the size of the sketch data structure for each vertex is $O(\log^3\nodesize)$.  We refer to the sketch data structure for each vertex as a \defn{vertex sketch} and each of its $\log\nodesize$ $\ell_0$-subsketches as \cubesketch{}s. Since \graphzep is designed to run efficiently out-of-core, it modifies this iterated vertex merging process to be write-optimal~\cite{graphzeppelin}; we omit the details here because \sysname does not use this technique.

The total size of the entire sketch data structure for either algorithm is $O\nodesize \log^3(\nodesize)$. \graphzep's gutter tree structure also has size $O(\nodesize \log^3\nodesize)$. Recent work ~\cite{nelson2019optimal} has shown that this space is asymptotically optimal. Because their $\ell_0$ sketch algorithms are randomized and can sometimes fail, the connectivity algorithm may also fail (subject to the choice of randomness used for the sketches). However, they show that these algorithms succeed with high probability: \ie they fail to return the correct answer with probability at most $1/\nodesize^c$ for some constant $c\geq1$ ($c$ appears as a constant factor in the space).



==> appendices/rounds.tex <==
\section{\sketchname Experiment}
\label{app:rounds}

We experimentally confirm that our implementation of \sketchname achieves the success probability proved in Lemma~\ref{lem:7-wise-sketch}. 
The experiment is as follows: 
\begin{enumerate}
    \item We initialize an empty \sketchname column $C$ with a unique seed for a vector of length $n=2^{24}$
    \item We insert a single unique non-zero into $C$.
    \item We query $C$ and record whether or not the query succeeded.
    \item We repeat steps $2$-$3$ until the column contains $n$ non-zeroes.
    \item We repeat steps $1$-$4$ for $500$ trials
\end{enumerate}

% There is correlation between our data points across $z$ but not between trials. That is, for a given $z$, each Bernoulli trial is independent. 

Our implementation forgoes the additional depth-1 bucket $b^*_1$. For this reason, we omit the case of $z=2$ from our analysis.

Due to high correlation between $z$ values, we limit our analysis to counting the number of $z$ value-means that are above a given threshold. If a given $z$ value (or, more likely, a region of $z$ values) had a much different probability than other regions, this experiment would still likely catch it. This is because if two non-zero values are highly correlated then their probabilities of success must be very similar. By Bayes Theorem, if $P[A \mid B] \approx 1$ and $P[B \mid A] \approx 1$ then $P[A] \approx P[B]$. This experiment would also catch if xxHash is insufficient for use with \sketchname.

For all values $z$, the mean probability of success is greater than $0.76$. For $99\%$ of the $z$ values, their mean success probability was greater than $0.78$. Additionally, the standard deviation is less than $0.02$ for all $z$.

%$n=2^{24}$, 500 trials, tested every possible number of non-zeros $\forall z \in [n] P[\text{sketch on $z$ non-zeros is good}] \geq 0.78$. 

xxHash, our hash function of choice, provides no proofs of $k$-wise independence or uniformity. Nevertheless, these results indicate xxHash is sufficient for use with \sketchname.
%We experimentally show how many rounds of Boruvka's algorithm it takes \sysname to compute the connected components. We perform this experiment on the data sets from Table \ref{tab:datasets} as well as graphs representing a single unbroken path. For each graph, we ingest and compute the connected components, measuring the number of rounds required.

%The path graphs are randomly generated by permuting a vector of integers. The permutation determines the connectivity; adjacent integers represent adjacent vertices in the path. We compute 100 different path graphs and measure the number of rounds for each.

%For the Table \ref{tab:datasets} we re-ran the ingesting and computation of the connected components 100 times. Each measurement used different random state.



==> appendices/todo.tex <==
\section{FIGURE OUT WHERE EVERYTHING BELOW THIS GOES}
\evan{Everything after this is where I'm copying stuff from the paper that I trim down in the body}

\section{Sketching Graphs}
In this section we briefly review the prior work on connectivity sketching, and then present \sketchname, an improved sketching subroutine that reduces the update cost from $O(\log^2\nodesize)$ to $O(\log \nodesize)$, and reduces the sketch size by a significant constant factor ($73$\%).

\subsection{Prior Work}
Ahn \etal~\cite{Ahn2012} initiate the field of graph sketching with their connected components sketch, which solves the streaming connected components problem in $O(\nodesize \log^3\nodesize)$ space. A key subproblem in their algorithm is \defn{$\ell_0$-sampling}: a vector $x$ of length $n$ is defined by an input stream of updates of the form $(i,\Delta)$ where value $\Delta$ is added to $x_i$, and the task is to sample a nonzero element of $x$ using $o(n)$ space. They use an $\ell_0$-sampler (also called an $\ell_0$-sketch) due to Cormode \etal:

\begin{theorem} (Adapted from ~\cite{l0sketch}, Theorem 1):
Given a 2-wise independent hash family $\mathcal{F}$ and an input vector $x \in \mathbb{Z}^n$, there is an $\ell_0$-sampler using $O(\log^2(n)\log(1/\delta))$ space that succeeds with probability at least $1 - \delta$.
\end{theorem}

We denote the $\ell_0$ sketch of a vector $x$ as $\sketch(x)$.  The sketch is a linear function, \ie $\sketch(x) + \sketch(y) = \sketch(x+y)$ for any vectors $x$ and $y$. Ahn \etal define a \defn{characteristic vector} $\charvec_u \in \mathbb{Z}^{\nodesize^2}$ of each vertex $u \in \nodes$ such that each nonzero element of $\charvec_u$ denotes an edge incident to $u$. 
That is, $\charvec_u \in \{-1,0,1\}^{\binom{\nodesize}{2}}$ s.t. for all $0 \leq i < j < {\binom{\nodesize}{2}}$: 
$$\charvec_u[(i,j)] = \left\{ \begin{array}{ll}
            1 & \quad u = i \text{ and }(v_i, v_j) \in \edges \\
            -1 & \quad u = j \text{ and }(v_i, v_j) \in \edges \\
            0 & \quad \text{otherwise} 
            
        \end{array}\right\}%\{1$ $if$ $i = j$ $and$ $(v_j, v_k) \in E, -1$ $if$ $i = k$ $and$ $(v_j, v_k) \in E, 0 \text{ otherwise}\}
$$
Further, for any $S \subset \nodes$, the nonzero elements of $\charvec_S = \sum_{u \in S}\charvec_u$ are precisely the set of edges crossing the cut $S, \nodes \setminus S$. For each $u \in \nodes$, the algorithm computes $\sketch(\charvec_u)$: for each edge update $(u,v,\Delta)$ it computes $\sketch(x_u)$ and $\sketch(x_v)$ where $x_i$ denotes the vector with $1$ in position $i$ and 0 in all other positions. It maintains $\sketch(\charvec_u) = \sum_i \sketch(x_i)$ for each $u$. Then for arbitrary $S \subset \nodes$ they can sample an edge across the cut $S, \nodes \setminus S$ by computing $\sketch(\charvec_S) = \sum_{u\in S} \sketch(\charvec_u)$. This allows them to perform \Boruvka's algorithm using the sketches: they form $O(\log\nodesize)$ $\ell_0$-sketches $\sketch_0(\charvec_u), \sketch_1(\charvec_u), \cdots , \sketch_{O(\log\nodesize)}(\charvec_u)$ for each $u$. We call $\sketch(\charvec_u) = \bigcup_{i \in [O(\log\nodesize)]}\sketch_i(\charvec_u)$ the \defn{vertex sketch} of $u$, and it has size $O(\log^3 \nodesize)$. Then $\forall u \in 
\nodes$ they query $\sketch_1(\charvec_u)$ to sample an edge incident to $u$. For each resulting component $C$ they compute $\sketch_2(\charvec_C)$ and repeat until all connected components are found. By setting $\delta = 1/100$ they show that the algorithm terminates in $O(\log\nodesize)$ rounds w.h.p. In total, finding the connected components this way takes $O(\nodesize \log^2\nodesize)$ time. Since each vertex sketch $\sketch(\charvec_u)$ has size $O(\log^3\nodesize)$ bits, the entire data structure has size $O(\nodesize\log^3\nodesize)$.

\paragraph{Testing k-connectivity.}
AGM ~\cite{Ahn2012} also show how to test k-connectivity of a graph $\graph = (\nodes, \edges)$ (that is, to exactly compute the minimum cut of $\graph$ provided this value is $\leq k$) by constructing a k-connectivity certificate $H = \bigcup_{i \in [k]} F_i $ where $F_0, F_1, \dots, F_{k-1}$ are edge-disjoint spanning forests of $\graph$. $H$ has the property that it is $k'$-edge connected iff $G$ is $k'$-edge connected for all $k' \leq k$. They find each $F_i$ by computing $k$ connectivity sketches of $\graph$ in a single pass over the stream. After the stream, the first connectivity sketch is used to find $F_0$ and the edges of $F_0$ are deleted from the remaining $k-1$ connectivity sketches. The second connectivity sketch can now be used to get $F_1$, whose edges are subsequently deleted from the remaining $k-2$ sketches and so on. The size of the sketches is $O(k\nodesize\log^3\nodesize)$ bits.

\paragraph{\graphzep.}
Tench \etal~\cite{graphzeppelin} present \graphzep, the first implementation of Ahn \etal's connected components algorithm which uses a faster $\ell_0$-sketch algorithm which they call \cubesketch. We summarize it here and then present our improved algorithm \sketchname. We also note that \graphzep uses an external-memory-optimized data structure called a \defn{gutter tree} to I/O-efficiently collect updates to be processed, allowing the algorithm to run quickly even when the sketches are stored on disk.
%For more details on Ahn \etal and Tench \etal's algorithms see Appendix~\ref{app:alg}.

\input{figures/cube_sketch_api}
\paragraph{Summary of \cubesketch.} Given a vector $\charvec \in \mathbb{Z}_2^\veclength$, a \cubesketch consists of a matrix of $\log(\veclength)$ by $\log(1/\delta)$ \defn{buckets}.
%\gil{a \cubesketch contains a matrix made up of $\log(1\delta)$ \defn{columns} each containing $\log(\veclength)$ \defn{buckets}}
Each bucket lossily represents the values at a random subset of positions of $\charvec$. It does so with two values \defn{$\indexsubset.\alpha$}, which is the xor of all nonzero positions, and \defn{$\indexsubset.\gamma$}, the xor of the hash of each nonzero position.  We can recover a nonzero element of $\charvec$ from bucket $\indexsubset_{i,j}$ only when a single position in $\indexsubset_{i,j}$ is nonzero. In this case we call bucket $\indexsubset_{i,j}$ \defn{good}, otherwise we say it is \defn{bad}. When $\indexsubset$ is good, then $\indexsubset.\alpha$ is equal to the nonzero index and $\text{hash}(\indexsubset.\alpha) = \indexsubset.\gamma$. If $\indexsubset$ is bad then with high probability $\text{hash}(\indexsubset.\alpha) \not= \indexsubset.\gamma$. The procedure for updating index $i$ is outlined in Figure~\ref{fig:cube_code}: for each column $c$, row $r$ is chosen with probability $1/2^r$ (using a $2$-wise independent hash function $h_j: [n] \rightarrow \log\veclength$) and $i$ is applied to each $b_{j,c}$ for $j \leq r$.
%\begin{theorem}[Restated from~\cite{graphzeppelin}]
\evan{We need to decide upon non-colliding variables for $\alpha$ and $\gamma$}
% \begin{restatable}[Adapted from ~\cite{graphzeppelin}, Theorem 1]{theorem}{cubesketchthm}
% \cubesketch is an $\ell_0$ sampler that, for vector $x \in \{-1,0,1\}^n$, uses $O(\log^2(n)\log(1/\delta))$ space, has worst-case update time $O(\log(n)\log(1/\delta))$, and succeeds with probability $1-\delta$.
% \end{restatable}

%\label{thm:cubesketch}
%\cubesketch is an $\ell_0$ sampler that, for input vector $x \in \mathbb{Z}_2^\veclength$, has space complexity $O(\log^2(\veclength)\log(1/\delta))$, worst-case update complexity $O(\log(\veclength)\log(1/\delta))$, average-case update complexity $O(\log(1/\delta))$, and failure probability at most $\delta$.
%\end{theorem}

To achieve a failure probability of $\delta$, \cubesketch uses $O(\log^2(n)\log(1/\delta))$ space and has worst-case update time $O(\log(n)\log(1/\delta))$.
In both \graphzep and \sysname, $\delta = 1/100$ and $O(\log\nodesize)$ sketches are maintained for each vertex sketch. The  vertex sketch update complexity is thus $O(\log^2\nodesize)$ when using \cubesketches, but will only be $O(\log \nodesize)$ when using \sketchnames.

\subsection{\sysname's new sketch: \sketchname}
% \label{subsec:cameo}
\input{figures/cameo_sketch_api}
We develop a new $\ell_0$ sampler called \sketchname for use in \sysname. \sketchname improves upon \cubesketch with a new update procedure that is a factor $\log n$ faster to update and reduces space usage by a constant factor via a refined analysis. All other details, including the query procedure, remain unchanged.

\paragraph{Update procedure.} \sketchname maintains the same matrix of buckets as \cubesketch, but uses a simpler and faster update procedure as shown in Figure~\ref{fig:cameo_code}. When performing an update $u$, for each column $c$ we choose a row $r$ independently with probability $1/2^r$. Unlike \cubesketch which updates all rows $[0, r]$ in the column, we apply $u$ to only $b_{0,c}$ and $b_{r,c}$. 

It is straightforward to see that \sketchname maintains the correctness and probabilistic bounds of \cubesketch. Assuming they use the same hash functions, if a bucket is good in the latter it must also be good in the former.
% Furthermore, we maintain an additional independent bucket $b^*_{1, j}$ of depth one in each column. We update this bucket with probability $1/2$ for each update. 

% Since each \sketchname update requires a constant number of RAM operations per $\ell_0$ sketch, its update cost is $O(\log\nodesize)$.

\begin{theorem}
    % \label{thm:cameo_update}
    \sketchname is an $\ell_0$ sampler that, for vector $x \in \mathbb{Z}_2^n$, uses $O(\log^2(n)\log(1/\delta))$ space, has worst-case update time $O(\log(1/\delta))$, and succeeds with probability $1-\delta$.
\end{theorem}

Theorem~\ref{thm:cameo_update} demonstrates that \sketchname reduces the CPU burden of performing updates and supports Claim~\ref{claim:all}.\ref{itm:cpu}.

\paragraph{Reduced constant factors.} In \graphzep, Tench \etal use $72 \log (1/\delta)\log n$ bytes of space to guarantee a failure probability of at most $\delta$ when sketching a vector of length $n < 2^{64}$ using \cubesketch. Via a careful constant-factor analysis, we can show that \sketchname can match this failure probability with significantly less space: 
%\paragraph{Correctness.} If a \cubesketch query succeeds, it does so because some bucket $b_{i,j}$ is good; it contains only one update $u$. 
%Note that $b_{k,j}$ is bad $\forall k \neq i$. 
%If \sketchname and \cubesketch use the same randomly chosen hash functions (and therefore select the same $i$ for each column $j$ for each update $u$), then \sketchname applies $u$ to a subset of the buckets that \cubesketch does. Therefore, if a \cubesketch query succeeds for a given input stream, then a \sketchname query will succeed as well. \evan{Somewhere in the rewrites this became unconvincing. Make better}\david{correctness is whp and relies on having the same number of columns as cubesketch and using the same query algorithm. we just need to redo correctness from scratch i think (and therefore explicitly use 2 universal hash functions}


%\gil{probably put the special 2 case thing here!! ! }

\begin{restatable}{theorem}{cameospacethm}
    % \label{thm:cameo_cols}
    Using $7$-wise independent hash functions, \sketchname requires $12\log_{9/2}(1/\delta) (\log n + 5)$ bytes of space to return a nonzero element of a length $n < 2^{64}$ input vector w/p at least $1-\delta$.
\end{restatable}

The intuition behind this result is that for every sketch column there exists a depth $d$ such that fewer than 7 of the stored elements exist below it. Given this knowledge, we can use fully independent analysis upon this subset of the buckets to achieve a tighter lower bound on the probability of success.
We omit the complete proof due to space constraints. 
% \evan{I really worry about not supporting this Theorem at all. If we can somehow fit a portion of Daniel's experiments that would help. Or even just a few sentences of intuition would make a big difference.}

Theorem~\ref{thm:cameo_cols} immediately implies a space savings of up to 92\% compared to \cubesketch and thus supports Claim~\ref{claim:all}.\ref{itm:space}. In our implementation, we conservatively choose to use slightly more space than this theorem requires to reduce the failure probability further. Still, our implementation requires only $2/7$ths of the space used in \graphzep~\cite{graphzeppelin} (see Section~\ref{sec:system} for details).

==> batches_old.tex <==
\subsection{Vertex-Based Batching}
\label{subsec:batch}

The core technique that makes distributed sketch processing efficient is \emph{vertex-based batching}, where many updates with a common endpoint are collected into a batch and sent to a single distributed worker for processing. 

To see why vertex-based batching is necessary (though not sufficient on its own) to minimize network communication, consider a simpler approach to distributing the sketch updates: An edge update $(u,v)$ requires updating the \sketchnames for vertices $u$ and $v$ (as in Section~\ref{subsec:alg}). Let $u_t$ be the adjacency list of $u$ at time $t$, and let $i$ be an update that arrives at time $t$ and has $u$ as one of its endpoints. By linearity, $\sketch(u_t + i) = \sketch(u_t) + \sketch(i)$ where $\sketch(x)$ denotes the \sketchname for the adjacency list of vertex $x$.  So a distributed worker can receive update $i$, compute $\sketch_u(i)$, and send it to the main node where it is added to $\sketch(u_t)$.

However, there are several problems with this naive approach. First, the latency costs of sending an individual network message for each edge update in the input stream are prohibitive. Edge updates from the input stream must be collected into batches to amortize the latency of network communication. Second, if each batch simply consisted of some contiguous subsequence of the input stream, in the worst case (and the average case) none of the updates in the batch will have endpoints in common.  In this case after processing the updates the distributed worker must send a sketch of size $\sketchsize = O(\log^3(\nodesize))$ bits \emph{for each update in the batch} back to the main node.  

To avoid this $O(\log^2(\nodesize))$-factor communication overhead, each batch sent to a distributed worker must contain only contain updates which share a common endpoint $u \in \nodes$ --- in other words, it must be a vertex-based batch. If a batch has this property, the distributed worker only needs to send a single sketch back to the main node. Provided the batch is of size $\alpha\times \sketchsize)$ for some constant $\alpha\geq1$, the overall communication cost per update remains constant.

Say the stream contains $\streamlength$ updates. The bandwidth cost to receive the input stream is $\streamlength$. Since each update is included in two vertex-based batches (one per endpoint) and each batch is sent to a distributed worker once, the total bandwidth cost of sending vertex-based batches is $2\streamlength$. Finally, each vertex-based batch induces the distributed worker that receives it to respond with a sketch delta (which is $1/\alpha$ of the batch's size). This gives us the following lemma:

\begin{lemma}
\label{thm:ingest}
Assuming no connectivity queries are issued, and $\edgesize = \Omega(\nodesize\log^3(\nodesize))$, the network bandwidth cost of ingesting $\streamlength$ updates is at most $(3 + 1/\alpha) \streamlength$.
\end{lemma}

==> figures/buffer.tex <==
\begin{figure}
    \centering
    \includegraphics[width=.45\textwidth]{figures/images/buffer.png}
    \caption{GraphZeppelin's gutter tree fails to scale beyond 70 million updates/sec. \sysname's pipeline hypertree can buffer stream updates at more than 500 million u/s.}
    \label{fig:buffer}
\end{figure}

==> figures/network.tex <==


\begin{figure}
\centering
\begin{subfigure}{0.45\textwidth}
    \includegraphics[width=\textwidth]{figures/images/throughput.png}
    \caption{Network message throughput vs batch size.}
    \label{fig:network_throughput}
\end{subfigure}
\hfill
\begin{subfigure}{0.45\textwidth}
    \includegraphics[width=\textwidth]{figures/images/latency.png}
    \caption{ Network message latency vs batch size.}
    \label{fig:network_latency}
\end{subfigure}

        
\caption{\sysname's message passing policy maximizes bandwidth use and amortizes away latency costs.}
\label{fig:network}
\end{figure}


==> figures/network_latency.tex <==
\begin{subfigure}
    \centering
    \includegraphics[width=.45\textwidth]{figures/images/latency.png}
    \caption{Network message latency vs batch size.}
    \label{fig:network_latency}
\end{subfigure}

==> figures/network_throughput.tex <==
\begin{subfigure}
    \centering
    \includegraphics[width=.45\textwidth]{figures/images/throughput.png}
    \caption{When \sysname sends  3000-10000 updates per vertex-based batch to each distributed worker, it reaches the half-bandwidth point: the message latency is amortized across the updates Network message throughput vs batch size.}
    \label{fig:network_throughput}
\end{subfigure}

==> figures/query.tex <==
\begin{figure}
    \centering
    \includegraphics[width=.45\textwidth]{figures/images/query.png}
    \caption{Most of the latency for connectivity queries is due to the need to flush and process pending updates before running Boruvka's algorithm to compute connectivity.}
    \label{fig:query}
\end{figure}

==> figures/query_gz.tex <==
\begin{figure}
    \centering
    \includegraphics[width=.45\textwidth]{figures/images/dsu_query_gz.png}
    \caption{\sysname's opportunistic query elision leads to lower latency for bursty queries than GraphZeppelin.}
    \label{fig:query_gz}
\end{figure}
%\vspace{-20em}

==> figures/scaling_comm.tex <==
\begin{figure}
    \centering
    \includegraphics[width=.45\textwidth]{figures/images/scaling_comm.png}
    \caption{The amount of network communication \sysname uses says constant as more worker nodes are added.}
    \label{fig:scaling_comm}
\end{figure}

==> figures/spark.tex <==
\begin{figure*}
\begin{center}
%\def\arraystretch{1.1}
\begin{tabular}{ |c|c|c|c|c|c| } 
 \hline
 Dataset & File Ingestion (s) & Create Frame(s) & CC time (s) & Total time (s) & Communication (as a factor of graph size)\\ 
 \hline
 \textbf{kron13} & 1.45 & 2.01 & 23.9 & 40.7 & 12.6\\
 \hline
 \textbf{kron15} & 43.8 & 5.11 & 34.7 & 95.5 & 4.44\\ 
 \hline
 \textbf{kron16} & 180 & N/A & N/A & $>5400$ & 11.1\\ 
 \hline
 
\end{tabular}
\end{center}
%\setlength{\belowcaptionskip}{-16pt} 
\caption{Spark's distributed GraphX connected components algorithm incurs significant overheads when processing dense graphs.}
\label{tab:spark}
\end{figure*}


==> intro_old.tex <==
\section{Introduction}
% using sysbench

Computing connected components\david{this stuff actually needs to change because we need to talk about k connectivity too.} is a fundamental graph-processing task
with uses throughout computer science and engineering. It has applications in relational databases~\cite{sigmodconn1}, scientific computing~\cite{scientific_computing1,scientific_computing2}, pattern recognition~\cite{pattern1,pattern2}, graph partitioning~\cite{partition1,partition2}, random walks~\cite{randomwalks}, social network community detection~\cite{lee2014social}, graph compression~\cite{compression1,compression2}, medical imaging~\cite{tumor}, flow simulation~\cite{bioinformatics1}, genomics~\cite{metagenomics1,metagenomics2}, identifying protein families~\cite{protein1,bioinformatics2}, microbiology~\cite{cell}, and object recognition~\cite{object}.  Strictly harder problems such as edge/vertex connectivity, shortest paths, and $k$-cores often use it as a subroutine, and it is used as a heuristic for clustering problems, ~\cite{clustering1,clustering2,clustering3,clustering4,clustering5,clustering6}, pathfinding algorithms such as Djikstra and $A^*$, and some minimum spanning tree algorithms. A survey by Sahu \etal~\cite{ubiquitous} of industrial uses of algorithms reports that, for both practitioners and academic researchers, connected components was the most frequently performed computation from a list of 13 fundamental graph problems that includes shortest paths, triangle counting, and minimum spanning trees.

\newtext{
Computing the minimum cut of a graph is a closely related problem to connectivity. It has applications in graph drawing~\cite{kant1993algorithms}, network reliability~\cite{ramanathan1987counting,karger1995randomized}, and VLSI design~\cite{krishnamurthy1984improved}.
}

The task of computing connected components becomes more difficult when graphs are \defn{dynamic}, meaning the edge set changes over time subject to a stream of edge insertions and deletions, and this task becomes harder still when the graphs are very large. Applications using dynamic graphs include identifying objects from a video feed rather than a static image~\cite{movingobject} or tracking communities in social networks that change as users add or delete friends~\cite{dynamic_social,dynamic_web}. Applications on large graphs include metagenome assembly tasks that may include hundreds of millions of genes with complex relations~\cite{metagenomics1}, and large-scale clustering, which is a common machine learning challenge~\cite{clustering3}.  And of course graphs can be both large and dynamic.  Indeed, Sahu \etal's~\cite{ubiquitous} survey reports that a majority of industry respondents work with large graphs ($> 1$ million verticess or $> 1$ billion edges) and a majority work with dynamic graphs.

%\david{we are trying to show: 1) we're different than GraphZeppelin. we overcome things they don't. there are fundamental differences. 2) we overcome these 3 bottlenecks and this is simultaneously surprising, impressive, and believable. 3) this is possible because linear sketching}
\paragraph{Dense-graph processing.} 
The task of computing connected components is especially
difficult for dynamic
\defn{dense graphs}.
%
%Also difficult for graphs that are large and dense. 
The conventional wisdom is that massive graphs are always sparse, meaning that they have few edges per vertex. Tench \etal~\cite{graphzeppelin} argue that large, dense graphs do exist but they are rarely studied due to a selection effect: most dynamic graph-processing techniques require storing the graph explicitly in RAM and therefore run out of memory on massive dense graphs.
%Their case for studying large dense graphs includes (1)~ an analysis of the density of graphs in publicly available repositories of graph datasets~\cite{netrepo, snapnets},
Their case for studying\david{michael doesn't like this phrasing} large dense graphs includes mentions of dense graphs in publications by industrial researchers, including for example, Facebook ad-recommendation tasks~\cite{facebookdense}. 

% \paragraph{Linear sketching for large dense graphs.}
Tench \etal  demonstrate that \defn{linear
sketching} techniques 
can be used to process large, dense, dynamic graphs\david{comma comma comma comma comma consistencyyyyyy you come and goooooo}. Linear sketching is most effective\david{beneficial? advantageous?} when graphs are dense---this is because
the size of a connectivity sketch is $O(\nodesize \polylog(\nodesize))$\david{define V} and therefore
is independent of the number of edges. 

However, the price for the small space of the sketches is high CPU cost: processing each update requires $O(\log^2(\nodesize))$ work, and the constants hidden by the asymptotic notation are large. Concretely, for a million-vertex graph, processing each edge \defn{update} (an insertion or deletion) requires evaluating roughly 500 hash functions (in addition to other costs). Their\david{been too long for this pronoun} implementation, \graphzep, introduces some techniques for mitigating this high computational cost but ultimately they are still bottlenecked by CPU.\david{ending on a down note - say what the tradeoff is: the CPU cost is the price of amazing space savings.}
%partially addresses this high CPU cost by parallelizing the updates but ultimately they are limited by the number of cores on a single machine and so \graphzep is CPU bound.


%Their tradeoff: reduced space cost. But intensive CPU cost because updating the sketches is computationally expensive. Although the update cost grows slowly---just $O(\polylog (V)$---this means that updates are fully bottlenecked on CPU, even though the sketches are small enough that graphs can be managed.

%the only hope for this being fast enough is parallelism, but they quickly exhausted the parallelism available on a single machine. so they're still CPU bound

%\paragraph{This paper.} In this paper we show how to attain the space savings of linear sketching for connected components without suffering from the CPU bottleneck. We accomplish this by distributing the work of updating the sketches to a cluster, exploiting the data locality and reduced total work of a new sketch algorithm to minimize the network communication costs across the cluster.

\paragraph{This paper.} We propose and implement a distributed sketching algorithm for the dynamic connected components problem.  We compute dynamic connected components in small space via sketching (as does \graphzep). 
The surprise is that we can get around the CPU bottleneck despite the inherently computation-intensive nature of sketching.  
We avoid the CPU bottleneck by distributing the work of processing sketch updates across many workers in a cluster. 

But we now have a distributed graph problem, and distributed graph-processing systems are notoriously bottlenecked on communication cost. 
Surprisingly, our system's communication costs can be amortized away to the point that they are not the bottleneck either.
(In fact, the bottleneck is the cost to process incoming edges on the main node, which we define below, and the limiting resource is sequential RAM bandwidth.)


Before we present our results in greater depth,
we explain the bottlenecks in graph-stream processing, and how they affect existing graph-processing systems.


%Linear sketching techniques have been applied in many contexts to scalably process large, dynamic datasets because they use very small space and can handle insertions and deletions to data. Prior to this work, linear sketching was not used for graph processing despite the fact that there is a rich theory literature on graph sketching. Recent work~\cite{graphzeppelin} gave linear sketching algorithms for finding connected components of graph streams, drastically reducing the cost of processing large, dense graphs. In addition to demonstrating that linear sketching methods are useful for large-scale graph processing, this work motivated the need for processing large, dense graphs, in contrast to most prior graph processing systems which optimize for sparse graphs.



\subsection{Three Bottlenecks in Graph-Stream Processing}
Graph-stream processing systems can be bottlenecked on any of three resources: \defn{space}, \defn{CPU}, and \defn{communication}. Even single-worker systems require some network communication; at minimum they must receive the input stream from a network link.

Some systems, such as Aspen~\cite{aspen} and Terrace~\cite{terrace}, are bottlenecked on \defn{space}. These systems maintain lossless representations of the input graph in RAM on a single machine, and such lossless representations can be large.  These systems are optimized for processing sparse graphs where this memory burden is less onerous but struggle when processing large, dense graphs.

Other 
systems, such as GraphZeppelin~\cite{graphzeppelin}, are bottlenecked on \defn{computation} (as we explain earlier).  GraphZeppelin maintains a lossily-compressed graph representation, reducing storage requirements (and improving performance on dense graphs) at the cost of higher CPU load for processing updates and  answering
%computing 
queries.

Distributed graph-stream processing systems are bottlenecked by network \defn{communication}. The input stream is received at a central node called the \defn{main node} and information about the graph is distributed across the cluster to \defn{worker nodes}. Since the graph data is spread across many worker nodes, and graphs often have poor data locality, most computation on graphs require worker nodes to send lots of information to each other~\cite{kineograph,graphtau,kickstarter,iyer2015celliq,iyer2021tegra,distinger}.  This is an example of a general challenge in distributed database systems.  These systems scale by spreading data among the aggregated memory of nodes in a cluster at the cost of high inter-node communication, which can increase query and transaction latencies~\cite{scalestore,dragojevic2014farm,Dragojevic2015NoCD}.


\input{figures/report_card}

Table~\ref{tab:report_card} summarizes the bottlenecks for each of these approaches. 

\paragraph{Objective standard for update performance: RAM bandwidth.} 
The update performance of any graph-streaming system is limited by the \defn{data acquisition cost}, that is, the cost for the master node simply to read the entire input stream. Even if we ignore the cost to update the connectivity information in the graph data structures, we still need to read the input. Thus, an objective standard describing the ideal performance is simply the RAM bandwidth. 
In fact, there are two notions of RAM bandwidth: \defn{random-access RAM bandwidth} (the speed at which we can write words to random locations) and 
\defn{sequential-access RAM bandwidth} (the speed at which we can write words to sequential locations). 

Since graphs have notoriously poor data locality, an update rate close to random-access RAM bandwidth is a natural goal for a graph stream-processing system.
Sequential-access RAM bandwidth is truly a bound on the best possible update rate because any stream-processing system must write the input data into memory, that is, must pay the data acquisition cost.
%Receiving the input stream at the main node, for any graph-stream processing system, has a RAM-bandwidth cost, which we call the \defn{data acquisition cost}. Since any such system must at least write the input stream in RAM, the rate at which the stream is processed is bounded above by sequential RAM bandwidth: the maximum rate at which the CPU can write consecutive words in RAM. Since graphs have poor data locality, it seems challenging (though not obviously impossible) for a system to exceed random-access RAM bandwidth.

\subsection{The \sysname Graph-Processing System}

In this paper we present \sysname, a linear-sketch-based distributed graph-stream processing system that computes connected components of dynamic graphs. 

\paragraph{\sysname's design overcomes the bottlenecks.}
\sysname keeps its sketch (a lossily compressed graph representation) on the main node and distributes the CPU work of processing updates. 

% \paragraph{System structure.}
Because these linear sketches are small (size $\Theta(\nodesize\log^3(\nodesize))$), they fit on a single node, even when the graph is dense.
The work to maintain these sketches can be chunked off into large batches  that can be computed independently by worker nodes. 
As a result, \sysname avoids the CPU bottleneck because it has lots of worker nodes to help, and \sysname avoids the communication bottleneck because the communication cost is amortized away by the CPU cost to process a batch. 
%\sysname avoids the CPU and communication bottlenecks of existing graph-stream processing systems.  

In fact, for any sequence of graph updates and queries 
\sysname's total communication cost is only a (small) constant factor larger than the cost for the main node to receive the input stream. 
Additionally, \sysname uses a new sketching algorithm, \sketchname, which requires only $O(\log(\nodesize))$ work per update (compared to $O(\log^2(\nodesize))$ for the prior state of the art).

% We compare \sysname's approach with other approaches for graph-stream processing from an asymptotic perspective in Table~\ref{tab:report_card}. 


% asymptotic performance is summarized in Table~\ref{tab:report_card}. 
%\sout{Therefore \sysname is not bottlenecked on any of the traditional resources and instead exposes another bottleneck.}
%the absolute minimum communication required (\ie the network bandwidth required to receive the input stream at the main node).  

\begin{comment}
\paragraph{Objective standard for performance.}
There is in fact an objective standard for ideal performance for a dynamic graph any streaming system.
Specifically, the RAM bandwidth of the main node. 
This is because in any system where you have a main node and worker nodes, all of the graph updates arrive at the main node. Even if we fully ignore the cost of processing these updates, we still need to write down the edges in ram at the main node.
\mab{just for what it's worth, note that we are using the word node in two different ways. One to meet vertex. The other to mean worker. We want to get rid of this ambiguity. }

In fact, RAM bandwidth can mean two different things... 
(1) sequential ram bandwidth, where we are sequentially writing data in ram. 
(2) random-access ram bandwidth, which is... 




Write something fast there's some sort of idealized version four Grass performance, which is the

Ram bandwidth just redo this cause this is total crap
\end{comment}

\paragraph{Performance.}
\sysname achieves the following:
% remarkable performance:
\begin{itemize}[noitemsep,topsep=0pt,leftmargin=*]
    \item \sysname is able to process graph streams only $4.5\times$ slower than the multi-threaded RAM sequential-write bandwidth, the objective upper bound on insertion performance for any system that receives the input stream at the main node. This is more than four times faster than random access RAM bandwidth.
    \item We show that \sysname can ingest up to 332 million stream updates per second on a graph with $2^{17}$ vertices.
    \item We show that it scales well with more distributed compute power: given a cluster of 40 distributed worker machines, it can ingest updates 35 times as fast as with 1 distributed worker machine.
    \item We experimentally verify that \sysname uses at most $4\times$ the network bandwidth required to read the input stream.
    \item Even on a single node, \sysname achieves an order of magnitude higher ingestion throughput than \graphzep, the prior state-of-the-art.
    \item Our  \dsuname query algorithm is capable of heuristically reusing partial information from prior query results, achieving up to a four orders-of-magnitude reduction in query latency over \graphzep.
\end{itemize}   

Table~\ref{tab:report_card} summarizes: \sysname is not bottlenecked on space, CPU, or communication.

%\paragraph{Revisiting objective standard for update performance and data structure size: adjacency matrices and RAM bandwidth. And so forth and so on. Cook until done. Lather rinse repeat.}
\paragraph{Outperforming lossless representations.}
To put this performance in context, consider a simpler task: maintaining an adjacency matrix of the graph defined by the input stream.
If the graph is dense and edges are random, an adjacency matrix is essentially the space-optimal lossless graph representation. 
We ignore the cost of answering queries, which an adjacency matrix does not efficiently support.

\sysname's graph-sketch representation is smaller than this adjacency matrix. Even more impressively \sysname's update throughput is also faster than the update throughput of the adjacency-matrix representation---which is just a single bit flip per edge.  
We emphasize: distributed \sketchname updates are faster than adjacency-matrix updates even when the entire adjacency matrix fits in RAM. 

\sysname's updates are fast not because they are small, but because the \sketchnames have good data locality---and the edge updates result in primarily sequential accesses to RAM on the main node, rather than random access.
%In fact, surprisingly, we process edge updates even faster than  the random-access RAM bandwidth. 
Said differently, we process more edge updates per second than it is possible to flip bits in random locations in RAM.
%\mab{Does this fix concerns about units? I'll explain when we talk}
%In fact, as we explain below, our update costs are within a factor of $4\times$ the cost of simply writing down the edge updates sequentially in RAM. 
And we perform these fast edge updates while actually supporting fast queries.

%To contextualize this result,
%To put this result in context, just receiving the input stream at a main node -- for \sysname or any other system -- has a RAM-bandwidth cost, which we call the \defn{data acquisition cost}, and \sysname is within a factor of 8 of this cost.  \david{Michael asks if there's a factor 2 to our advantage here because in a distributed system you have to write the data and then read it again when you're sending to worker nodes.} Furthermore,\david{michael says this isn't a furthermore, it's additional context for the same number - how goshdarn fast we are.} \sysname can process graph streams more than twice as fast as random-access RAM bandwidth (the maximum rate at which the CPU on the main node can write to nonsequential words in RAM using any number of threads). 
%\mab{Given that graphs generally have poor data locality, it's almost believable that we can stream graphs faster than the random access ran band width. Following sentence is not quite right, since it's irrelevant about whether it's easy or difficult.}
%\mab{one more point: it feels as though we should present the ram bandwidth earlier than now. Specifically the fact that there are two different numbers. We should do this in the introduction as soon as we mention RAM bandwith. }
%\mab{issue: rather than saying, ``landscape, achieves...''
%We should say ``there's this other objective standard, which is RAM bandwidth. And in fact, there are two notions of ram bandwidth depending on whether we are talking about sequential access or random acces''}
%Given the poor data locality of graphs, it is challenging for a system to exceed the random-access RAM bandwidth, even for graphs that fit on a single node.
%\dan{We should be clear here-- we mean the cost to write. ram read bandwidth is incredibly high, think like 150GB/s. Access=Write is the bottleneck}

%\mab{in the writing, can we explicitly the cost to read the graph stream without processing to the cost of maintaining the updates? It's somehow not said as clearly as it could be what we mean. I'd like to talk to David about this over the phone.}
\begin{comment}
In summary, there are three performance bottlenecks that we need to overcome \emph{simultaneously} to improve graph stream processing: space, CPU, and network communication. 
\sysname overcomes these bottlenecks in three stages:
%(1) first develop a space efficient lossy graph sketch. This reduces the space so much that even very large very dense graphs fit on a single compute node.
First, \sysname uses lossy graph sketching to reduce space so much that even very large, very dense graphs fit on a single compute node. Unfortunately, these sketches increase the CPU load over direct graph algorithms. 
%The result is that by reducing the space we actually hurt the CPU cost.
Second, \sysname addresses the CPU bottleneck by distributing the sketching work, but this shifts the bottleneck to communication.
%By having a large number of CPU nodes, we can then get the total CPU requirements under control.
Third, we introduce new batching and scheduling data structures that exploit the linearity of our sketching algorithms to increase data locality, amortizing away the network bottleneck.

As a result, \sysname is capable of ingesting dense graph streams only a factor 4.5 slower than sequential RAM bandwidth.
\end{comment}


\section{Technical Overview}
We give a brief overview of the techniques that allow \sysname to overcome the CPU, communication, and space bottlenecks.


\paragraph{Overcoming the CPU bottleneck.}
Prior systems using linear sketching algorithms are bottlenecked on CPU cost~\cite{graphzeppelin,l0sketch}.
\sysname overcomes this high CPU cost in two ways: First, via algorithmic improvements that lower the total work required to update the sketches, and second, by distributing this work to worker nodes in the cluster.

\sysname's \sketchname algorithm significantly reduces update cost. Existing algorithms for $\ell_0-$sampling~\cite{graphzeppelin,l0sketch} (the key sampling subroutine for connected components sketching), including the state-of-the-art \cubesketch, have worst-case update time $O(\log^2(\nodesize))$. \sketchname's update time is $O(\log(\nodesize))$, which we show experimentally leads to a $4\times$ speedup over \cubesketch.

\sysname scales well when given more distributed compute power: given 40 distributed workers (with 16 cores each), it can ingest updates $35\times$ faster than with 1 distributed worker (with 16 cores). \sysname's high scalability is a consequence of its linear sketches. \sketchnames have strong data locality, which we exploit for parallelism: there is one sketch for each vertex in the graph; processing a graph edge update $(u,v)$ requires updating only the sketches of its endpoints $u$ and $v$; and these updates can be performed independently of each other. Because the sketches are linear, the sketch update for $(u,v)$ can be computed on its own and later summed to the sketch of $u$. This means that the vast majority of the computation required to process $(u,v)$ can be performed before accessing the sketches for $u$ and $v$. \sysname exploits this independence to distribute the computational cost of these updates while storing the sketches on a single worker. 


\paragraph{Overcoming the communication bottleneck.}
For any sequence of graph updates and connectivity queries, the total communication \sysname uses to process the stream and answer each query is at most a $(3 + \epsilon)$ factor larger than the bandwidth required to read in the input stream at the main node. Since any stream-processing system must receive the input stream over a network link at the main node, \sysname is therefore a small constant factor away from the minimum possible communication for any distributed solution to the streaming connected components problem.

\sysname accomplishes this remarkable result by exploiting the data locality properties of its \sketchnames. First, it collects updates into \defn{vertex-based batches}, defined to be a batch of edge updates that share a vertex. This amortizes the communication cost of distributing updates. Each vertex-based batch is processed by a single distributed worker. In Section \label{subsec:pht} we describe how updates are batched using \sysname's \defn{\treename} and in Section \ref{subsec:gzcomp} show how the \treename can process the input stream into batches at 1/3 of sequential RAM bandwidth. Second, \sysname's \defn {batch distribution policy} assigns batches to workers such that queries frequently require no additional communication.
Since its sketches are stored entirely on the main node, if the sketch has processed all pending updates, the query can be computed locally with latency at most twice as high as the best single-machine graph-stream processing systems~\cite{aspen,terrace,graphzeppelin}. If some pending updates have not been processed, the batch distribution policy chooses whether to distribute this work or perform it locally. In Section \ref{subsec:queries}, we describe this batch distribution policy and prove that for any sequence of graph updates and connectivity queries, the total communication required to process the stream and answer each query is at most a $(3 + \epsilon)$ factor larger than the bandwidth required to read in the input stream. %The sequences that produce the worst-case performance are pathological and unlikely to occur in practice; we show experimentally in Section \ref{subsec:queryex} that queries incur negligible communication on realistic inputs. \david{this sounds like a weakener so we need to make it clear that we're talking about getting better performance than the guarantee in almost all real scenarios.}

In certain cases, \sysname can compute queries using no communication at all. \sysname's queries produce a certificate that summarizes connectivity information. \sysname can also be configured to answer further queries more quickly if this certificate is still valid, a technique we call \defn{opportunistic query elision}. It is often possible to locally update the certificate as new graph updates arrive to maintain correctness without repeating the full query algorithm from scratch. Queries answered via opportunistic elision require no network communication whatsoever. \sysname is capable of performing these local updates and monitoring the certificate for correctness. If the input stream introduces updates that violate correctness, the certificate is discarded and the next query is computed from scratch. We show experimentally in Section \ref{subsec:queryex} that this results in a four orders-of-magnitude decrease in query latency for a variety of simulated graph-update and query sequences.


\paragraph{Overcoming the space bottleneck.}
Because \sysname's linear sketches are asymptotically smaller than the graph, they fit on a single node, even when the graph is very large (\ie has many vertices) and is dense. In fact, recent work~\cite{nelson2019optimal} has shown that \sysname's $O(\nodesize \log^3(\nodesize))$ space cost (where $\nodesize$ is the number of vertices in the graph) is asymptotically optimal when computing connected components on a stream with edge insertions and deletions. 

This asymptotic space cost translates to an actual space savings at surprisingly small graph sizes. The most compact lossless representation of a dense graph is an adjacency matrix with a single bit per entry. \sysname uses less space than such an adjacency matrix even when the input graph only has a million vertices, and we demonstrate experimentally that \sysname can still process such graphs at a bandwidth of hundreds of millions of edges per second. \sysname's \sketchnames are 2.3 times smaller than the state-of-the-art \cubesketch used by GraphZeppelin~\cite{graphzeppelin}. 
Specifically, \sysname uses $246(\log^2(\nodesize) - \log(\nodesize))$B of space for a graph on $\nodesize$ vertices.

%\sout{We experimentally show that \sysname is bottlenecked by the data acquisition bottleneck of RAM rather than CPU computation or network communication: We add worker nodes until \sysname stops getting faster, then increase the RAM bandwidth and find that the system gets faster again. }


%\hrulefill




%\sout{This peeling process of removing bottlenecks allows \sysname to achieve strong bounds across several dimensions: the space cost is asymptotically optimal, and the work required for each update is $O(\log(\nodesize))$. The network bandwidth is within a small constant factor of optimal (the data acquisition cost), and each piece of work requires exactly one network round trip with no synchronization requirements. \sysname therefore achieves throughput that is limited only by the data acquisition cost of RAM.}

==> intro_very_old.tex <==
\section{Introduction}
% using sysbench

Computing connected components is a fundamental graph-processing task
with uses throughout computer science and engineering. It has applications in relational databases~\cite{sigmodconn1}, scientific computing~\cite{scientific_computing1,scientific_computing2}, pattern recognition~\cite{pattern1,pattern2}, graph partitioning~\cite{partition1,partition2}, random walks~\cite{randomwalks}, social network community detection~\cite{lee2014social}, graph compression~\cite{compression1,compression2}, medical imaging~\cite{tumor}, flow simulation~\cite{bioinformatics1}, genomics~\cite{metagenomics1,metagenomics2}, identifying protein families~\cite{protein1,bioinformatics2}, microbiology~\cite{cell}, and object recognition~\cite{object}.  Strictly harder problems such as edge/vertex connectivity, shortest paths, and $k$-cores often use it as a subroutine, and it is used as a heuristic for clustering problems, ~\cite{clustering1,clustering2,clustering3,clustering4,clustering5,clustering6}, pathfinding algorithms such as Djikstra and $A^*$, and some minimum spanning tree algorithms. A survey by Sahu \etal~\cite{ubiquitous} of industrial uses of algorithms reports that, for both practitioners and academic researchers, connected components was the most frequently performed computation from a list of 13 fundamental graph problems that includes shortest paths, triangle counting, and minimum spanning trees.

The task of computing connected components becomes more difficult when graphs are \defn{dynamic}, meaning the edge set changes over time subject to a stream of edge insertions and deletions, and this task becomes harder still when the graphs are very large. Applications using dynamic graphs include identifying objects from a video feed rather than a static image~\cite{movingobject} or tracking communities in social networks that change as users add or delete friends~\cite{dynamic_social,dynamic_web}. Applications on large graphs include metagenome assembly tasks that may include hundreds of millions of genes with complex relations~\cite{metagenomics1}, and large-scale clustering, which is a common machine learning challenge~\cite{clustering3}.  And of course graphs can be both large and dynamic.  Indeed, Sahu \etal's~\cite{ubiquitous} survey reports that a majority of industry respondents work with large graphs ($> 1$ million nodes or $> 1$ billion edges) and a majority work with graphs that change over time.

Recent work~\cite{graphzeppelin} gave algorithms for processing high-speed graph streams even when the graphs are large and dense. These algorithms implement practical linear-sketching techniques that drastically reduce the cost of processing large, dense graphs. 
This work also motivates the need for such graph-processing systems.
%, since They additionally observed that large, dense graph datasets are analy noted a need for systems that optimize for processing large, dense graphs, citing the existence of such graphs as proprietary datasets analyzed at great cost by large corporations such as Facebook \cite{facebookdense}. Despite the fact that such large, dense graph datasets exist, they are rarely studied in the graph processing literature and do not appear in graph dataset repositories, indicating that researchers and engineers lack the tools required to process them.\david{michael: high order bit is that we can now process large dense graphs. secondary is that this matters}

Perhaps surprisingly, many of the fastest streaming graph-database systems store their graph representations and perform their computations on a single machine, and as a result are bottlenecked by both space and computation costs.
%Of course, a single machine's fixed-size memory is a fundamental bottleneck: larger graphs require more memory to represent.  Similarly, the machine's fixed processing power limits the speed and scale at which it can process graph streams.  Existing systems tend to be bottlenecked by one (or both) of these concerns.  
For example, some systems, such as Aspen~\cite{aspen} and Terrace~\cite{terrace}, maintain lossless representations of the input graph, which can be very large.  They are optimized for processing sparse graphs where this memory burden is less onerous but struggle when processing large, dense graphs. 
Other systems, such as GraphZeppelin~\cite{graphzeppelin}, are primarily bottlenecked by computation.  GraphZeppelin maintains a lossily-compressed representation of the graph, reducing storage requirements (and improving performance on dense graphs) at the cost of higher CPU load for processing updates and computing queries. 


These space and computation bottlenecks have motivated the creation of systems that distribute graph data and computation across many computers in a cluster.
%Systems that distribute their graph data across multiple compute nodes can overcome these space and computation bottlenecks but introduce a new bottleneck: communication costs. 
For existing distributed graph-processing systems, the input stream is received at a central node called the \defn{main node} and information about the graph is distributed across the cluster to \defn{worker nodes}. Since the graph data is spread across many nodes, and graphs often have poor data locality, most computation on graphs require worker nodes to send lots of information to each other. For this reason, many distributed graph-stream processing systems are bottlenecked primarily by communication costs~\cite{kineograph,graphtau,kickstarter,iyer2015celliq,iyer2021tegra,distinger}. This is an example of a general challenge in distributed database systems. These systems scale by spreading data among the aggregated memory of nodes in a cluster at the cost of high inter-node communication, which can limit query and transaction latencies~\cite{scalestore,dragojevic2014farm,Dragojevic2015NoCD}.
%even simple graph primitives like finding the neighbors of a vertex can require significant communication. While adding more workers to the cluster increases the storage and computation power available, it also increases the amount of communication required.  Indeed, many modern static and streaming graph-processing systems have high communication costs, which limit their scalability \cite{distributed_graph_systems}.

In this paper we present \sysname, a linear-sketch-based distributed graph-stream processing system that computes connected components of dynamic graphs. \sysname keeps its graph sketch (a lossily compressed graph representation) on the main node and distributes the CPU work of processing sketch updates. 
Because these linear sketches are asymptotically smaller than the graph, they fit on a single node, even when the graph is very large (\ie has many nodes) and is dense.
Furthermore, the work to maintain these sketches can be chunked off into large batches of work that can be computed by worker nodes. 
As a result, \sysname avoids the communication bottleneck because the communication cost is amortized away by the CPU costs, and \sysname avoids the CPU bottleneck because it has lots of worker nodes to help.
%\sysname avoids the CPU and communication bottlenecks of existing graph-stream processing systems.  
It is able to distribute the CPU work of graph-stream processing with minimal communication overhead: in fact, for any sequence of graph updates and queries we prove that \sysname's total communication cost is only a (small) constant factor larger than the cost for the main node to receive the input stream.
%the absolute minimum communication required (\ie the network bandwidth required to receive the input stream at the main node).  

As a result, \sysname achieves the following remarkable performance: it is able to process graph streams only $8\times$ slower than the multi-threaded RAM sequential-write bandwidth (the maximum rate at which the CPU on the main node can write consecutive words in RAM using any number of threads). 
%To contextualize this result,
To put this result in context, just receiving the input stream at a main node -- for \sysname or any other system -- has a RAM-bandwidth cost, and \sysname is within a factor 8 of this cost.  Furthermore, \sysname can process graph streams more than twice as fast as random-access RAM bandwidth (the maximum rate at which the CPU on the main node can write to nonsequential words in RAM using any number of threads). 
Given the poor data locality of graphs, it is challenging for a system to exceed the random-access RAM bandwidth, even for graphs that fit on a single node.
%\dan{We should be clear here-- we mean the cost to write. ram read bandwidth is incredibly high, think like 150GB/s. Access=Write is the bottleneck}

%\mab{in the writing, can we explicitly the cost to read the graph stream without processing to the cost of maintaining the updates? It's somehow not said as clearly as it could be what we mean. I'd like to talk to David about this over the phone.}


\sysname scales well when given more distributed compute power: given 160 distributed workers (with 16 cores each), it can ingest updates $92\times$ faster than with 1 distributed worker (with 16 cores). We experimentally show that \sysname is bottlenecked by RAM bandwidth rather than CPU computation or network communication: We add worker nodes until \sysname stops getting faster, then increase the RAM bandwidth and find that the system gets faster again. 

\sysname's low communication costs and high scalability are consequences of its linear sketches. Prior implementations of similar linear sketching algorithms are CPU-bound~\cite{graphzeppelin,l0sketch}, limiting their scalability.\dan{It may be valuable to say why. CPU boundedness is something shocking; even with two citations, a sentence saying 'This is intuitively because sketching requires many hashes and has good data locality' would be compelling.}  \sysname's sketches have strong data locality, which we exploit for parallelism: there is one sketch for each node in the graph; processing a graph edge update $(u,v)$ requires updating only the sketches of its endpoints $u$ and $v$; and these updates can be performed independently of each other. Moreover, the vast majority of the computation required to process $(u,v)$ can be performed before accessing the sketches for $u$ and $v$. \sysname exploits this independence to distribute the computational cost of these updates while storing the sketches on a single worker, minimizing communication costs. 

Another strength of \sysname is that it can frequently compute queries without any additional network communication. Since its sketches are stored entirely on the main node, if the sketch has processed all pending updates, the query can be computed locally with latency at most four times higher than the best single-machine graph-stream processing systems~\cite{aspen,terrace,graphzeppelin}. If some pending updates have not been processed, \sysname may incur additional communication costs as it processes them. We prove that for any sequence of graph updates and connectivity queries, the total communication required to process the stream and answer each query is at most a $(3 + \epsilon)$ factor larger than the bandwidth required to read in the input stream. The sequences that produce the worst-case performance are pathological and unlikely to occur in practice; we show experimentally that on realistic inputs queries incur negligible communication.

\sysname can also be configured to reduce query latency further by opportunistically reusing partial results from prior queries if they are still valid. Once a query is computed from scratch, it is often possible to greedily update the query answer as new graph updates arrive to maintain correctness without repeating the full query algorithm from scratch. Queries answered via this method require no network communication whatsoever. \sysname is capable of performing these greedy updates and monitoring the data structure for correctness. If the input stream introduces updates that violate correctness, the partial results from the last query are discarded and the next query is computed from scratch. We show experimentally that this results in a four orders-of-magnitude decrease in query latency for a variety of simulated graph-update and query sequences.

%In summary, \sysname overcomes the computation and communication bottlenecks that limit the scalability of existing graph-stream processing systems. We prove that its communication cost is within a small constant factor of the minimum communication possible: the communication required to receive the input stream. This low communication overhead and the strong data locality of linear sketching allows \sysname to distribute the CPU cost of updating its sketches extremely efficiently: it runs $92\times$ faster with 160 distributed workers than it does with 1 distributed worker. As a result, it can process graph streams only $8\times$ slower than multi-threaded RAM sequential bandwidth.

%\hrulefill

In summary, there are three performance bottlenecks that we need to overcome \emph{simultaneously} to improve graph stream processing: space, CPU, and network communication. 
\sysname takes an unconventional and indirect route to addressing these bottlenecks:
%(1) first develop a space efficient lossy graph sketch. This reduces the space so much that even very large very dense graphs fit on a single compute node.
\sysname uses lossy graph sketching to reduce space so much that even very large, very dense graphs fit on a single compute node. Unfortunately, these sketches increase the CPU load over direct graph algorithms. 
%The result is that by reducing the space we actually hurt the CPU cost.
\sysname addresses the CPU bottleneck by distributing the sketching work, but this shifts the bottleneck to communication.
%By having a large number of CPU nodes, we can then get the total CPU requirements under control.
Finally, we develop a linear sketch algorithm for \sysname that exhibits data locality which allows it to amortize away the network bottlenecks.
%[work chunking is something that you can only do with graph sketching, not with regular graph algorithms. So while there's more work, it's chunkable.]
%The result is that we solve all three of these problems.

This peeling process of removing bottlenecks allows \sysname to achieve strong bounds across several dimensions: the space cost is asymptotically optimal, and the per-update work span is constant. The network bandwidth is within a small constant factor of optimal (the cost of receiving the input stream), and each piece of work requires exactly one network round trip with no synchronization requirements. As a result the bottleneck of the system is the speed at which data can be sequentially written to RAM.
%[in contrast, the natural way that you might think of dealing with the space issue is first to distribute across all the nodes. But doing so means that we still have CPU bottlenecks and latency bottlenecks, which seems really difficult to get rid of.

%A priori this seems like a strange path to take because we begin by not using all the space that is available on a large memory machine while simultaneously increasing the CPU cost. But this has the benefit that while we end up with more CPU work, it's work that is chunkable to overcome latency bottlenecks.]



%\hrulefill

%\paragraph{Paper Organization.} We begin in Section~\ref{sec:preliminaries} by defining some notation for graphs and graph streams, as well as notions of RAM bandwidth which we will use to measure the performance of \sysname in our evaluation. We also summarize existing sketch-based algorithms for graph stream connectivity. Using these algorithms as a starting point, in Section~\ref{sec:bandwidth} we outline \sysname's distributed sketching algorithm and prove that it uses at most a small constant fraction more network bandwidth than is required to read in the input stream. In Section~\ref{sec:system} we describe \sysname's implementation, and in Section~\ref{sec:experiments} we evaluate its performance experimentally. Finally in Section~\ref{sec:related} we survey related work in graph stream processing systems.




==> pipeline_trash.tex <==

\evan{Not sure where all this fits so just putting it in a big block here. Also its bad writing for now.}
\textcolor{red}{
To provide reasoning for why the \treename massively outperforms the GutterTree let us analyze the PRAM Exclusive Read Exclusive Write (EREW) performance of each method. The span and work of creating vertex-based batches from $m$ updates. In fact, we will prove bounds on span and work using the even stronger restriction that only one thread may touch a shared node of the tree at once.
}

\textcolor{red}{
In order to get the performance of the below Theorem we have to make the following modifications to the \treename algorithm. First, when an internal node at the lowest thread local level is flushed the thread in question scans the buffer to check if it can create a leaf sized batch of updates destined for the same leaf to directly remove from the tree. This prevents the adversary from limiting our parallelism by having a large majority of updates be routed to the same leaf. However, an adversary could still defeat this technique by having most or all of the updates be destined for a single shared internal node. We solve this issue with the second modification, when constructing the \treename we randomly permute the key-space. Then when inserting an update, we first compute its randomized key and insert a modified update to the tree. When a leaf fills we identify the true key by reversing the permutation.
}

\textcolor{red}{
Since the adversary does not have access to our randomness, the best they can achieve to to randomly pick heavy hitter keys with the hope of a collision. Collisions (2 heavy keys residing within the same shared internal node) reduce performance because insertions of these keys to the shared internal node are sequential and in general this cannot be rectified with the eager batch optimization. For the remainder of this analysis we will only consider these heavy keys as the number of updates to other keys must be lower order for the adversary to reduce our performance. Let $h$ be the number of heavy keys, $p$ the number of threads, and $s(x)$ denote the number of first shared level nodes that have $x$ heavy keys mapped to them. The adversary's goal is to minimize the following equation subject to $h \geq 1$
$$\sum_{x \geq 2} s(x) + \frac{s(1)}{h}p$$
}

\textcolor{red}{
Given $h$ heavy keys, we can compute the expected values of $\sum_{x \geq 2}s(x)$ and $s(1)$. From the birthday problem, $\sum_{x \geq 2} s(x)$ is the expected number of ``days'' that have two or more birthday's on them. While $s(1)$ is the number of days that have exactly one birthday on them.
}

\textcolor{red}{
\begin{theorem}
    \label{thm:pht_parallel}
    The \treename creates vertex-based batches from $m$ updates with worst-case expected span $O((\cachelinesize/\cachesize)^3 m\log_{\frac{\cachesize}{\cachelinesize}} \nodesize)$ and work $O(m \log_{\frac{\cachesize}{\cachelinesize}} \nodesize)$ in the PRAM EREW model.
\end{theorem}
}

==> preliminaries_old.tex <==
\section{Preliminaries \& Definitions}
\label{sec:preliminaries}

\paragraph{Graph Streaming.} In the \defn{graph semi-streaming} model~\cite{semistreaming1,semistreaming2} (sometimes just called the \defn{graph streaming} model), an algorithm is presented with a \defn{stream} $\graphstream$ of updates (each an edge insertion or deletion) where the length of the stream is $\streamlength$. 
Stream $\graphstream$ defines an input graph $\graph = (\nodes,\edges)$ with $\nodesize = |\nodes|$ and $\edgesize = |\edges|$.  The challenge in this model is to compute (perhaps approximately) some property of $\graph$ given a single pass over $\graphstream$ and at most $O(\nodesize \polylog(\nodesize))$ words of memory.  
Each update has the form $((u,v), \Delta)$ where $u,v \in \edges, u \neq v$ and $\Delta \in \{-1,1\}$ where $1$ indicates an edge insertion and $-1$ indicates an edge deletion.  Let $\streamelement_i$ denote the $i$th element of $\graphstream$, and let $\graphstream_i$ denote the first $i$ elements of $\graphstream$.  
Let $\edges_i$ be the edge set defined by $\stream_i$, i.e., those edges which have been inserted and not subsequently deleted by step $i$.  The stream may only insert edge $e$ at time $i$ if $e \notin \edges_{i-1}$, and may only delete edge $e$ at time $i$ if $e \in \edges_{i-1}$.



\begin{problem}[\textbf{The streaming Connected Components problem.}]
Given a insert/delete edge stream of length $\streamlength$ that defines a graph $\graph = (\nodes, \edges)$, return a insert-only edge stream that defines a spanning forest of $\graph$.
\end{problem}

\begin{comment}

\paragraph{RAM bandwidth definitions.} We briefly define some notions of RAM and network bandwidth.

\begin{definition}[sequential and random-access RAM bandwidth]~~~
\begin{itemize}[leftmargin=*]
\item \defn{Single-threaded RAM sequential bandwidth} is the rate at which the CPU can write consecutive words in RAM on one thread. 

\item  \defn{Single-threaded RAM random access bandwidth} is the worst-case rate at which the CPU can write any sequence of words in RAM on one thread. 

\item \defn{Multi-threaded RAM sequential bandwidth} is the maximum rate at which the CPU can write consecutive words in RAM on any number of threads. 

\item We call the minimum number of threads that achieves this maximum rate to be the \defn{sequential RAM saturation point}.

\item \defn{Multi-threaded RAM random access bandwidth} is the maximum worst-case rate at which the CPU can write any sequence of words in RAM on any number of threads. 

\item We call the minimum number of threads that achieves this maximum rate to be the \defn{random RAM saturation point}.

%\item \defn{$k$-threaded RAM random access bandwidth} is the maximum rate at which the CPU can access a randomly chosen sequence of words in RAM on $k$ threads.  
    
\end{itemize} 

In any setting, we define the \defn{half-bandwidth point} to be the read or write granularity that is big enough to achieve half of the sustained bandwidth, so that half the time is spent setting up the transfer and half the time is spent transferring the data.

\end{definition}

\end{comment}

\paragraph{RAM bandwidth definitions.} We briefly define some notions of RAM and network bandwidth.

\begin{definition}[RAM bandwidth]~~~
\begin{itemize}[leftmargin=*]
\item \defn{RAM sequential bandwidth} is the maximum rate at which the CPU can write consecutive words in RAM on any number of threads. 

\item \defn{RAM random access bandwidth} is the maximum worst-case rate at which the CPU can write any sequence of words in RAM on any number of threads. 

%\item We call the minimum number of threads that achieves these rates to be the \defn{sequential RAM saturation point} and the \defn{random RAM saturation point}, respectively.

%\item \defn{$k$-threaded RAM random access bandwidth} is the maximum rate at which the CPU can access a randomly chosen sequence of words in RAM on $k$ threads.  
    
\end{itemize} 

In any setting, we define the \defn{half-bandwidth point} to be the read or write granularity large enough to achieve half of the sustained bandwidth, so that half the time is spent setting up the transfer and half the time is spent transferring the data.

\end{definition}




\begin{comment}
sequential access words on 1 thread, randomly accessing words on 1 thread, the above but multi threads.

Definitions: RAM latency is the time it takes after issuing a RAM read or write instruction for the read/write to finish.  RAM sequential bandwidth is how many bytes per second you can write to a contiguous region of memory.  RAM random access bandwidth is how many bytes per second you can write to a sequence of random locations in RAM.

\begin{itemize}
    \item \sysname ingestion rate within a small constant factor of RAM bandwidth. RAM bandwidth is 
    \item 
\end{itemize}

% !TEX root =  main.tex
\end{comment}



\paragraph{Prior Work in Connected Components Sketching.}
\label{subsec:alg}
\david{I've left a few paragraphs here to mockup the summary of the algorithm that will be here in the submitted version.}
Ahn \etal's~\cite{Ahn2012} presented \algname, the first connected components sketching algorithm (and indeed, the first linear sketch graph algorithm). Tench \etal's~\cite{graphzeppelin} later presented \graphzep, a connected components sketch which was additionally I/O optimal. At a high level, both algorithms create an \defn{$\ell_0$-sketch} of each graph vertex from which incident edges can be recovered. For each edge update $(u,v)$, the update is applied to the sketches for vertices $u$ and $v$. Using these sketches of the edges incident to each vertex, \algname and \graphzep use Boruvka's algorithm to compute connectivity. Each vertex sketch is $O(\log^3(\nodesize))$ bits, so the total sketch size is $O(\nodesize\log^3(\nodesize))$ which is optimal ~\cite{nelson2019optimal}. \graphzep additionally uses a \defn{gutter tree} to amortize data movement costs and achieve I/O optimality. See Tench \etal~\cite{graphzeppelin} for a detailed summary of these algorithms and their differences.


==> related_old.tex <==
\section{Related Work.}
\label{sec:related}
\paragraph{Single-Machine Streaming Graph Systems.}
Some single-machine streaming graph systems accept input streams with arbitrarily interspersed edge insertions, edge deletions, and queries~\cite{graphzeppelin,graphinc}.
Many existing single-machine graph stream processing systems are instead optimized for the \defn{batch-parallel} model where stream updates arrive in large batches consisting entirely of insertions or entirely of deletions. For many such systems larger batch sizes enable better performance. Some batch-parallel systems answer queries synchronously, meaning they stop ingesting stream updates while computing queries~\cite{terrace,busato2018hornet,ediger2012stinger,murray2016incremental,sengupta2016graphin,sengupta2017evograph}. Other allow periodically take ``snapshots'' of the graph during ingestion that enable asyncronous query evaluation during stream ingesion~\cite{aspen,cheng2012kineograph,iyer2015celliq,iyer2016time,macko2015llama}.
Some systems are designed to process only streams of edge insertions~\cite{jetstream,graphbolt}.

\begin{comment}
\paragraph{Distributed Static Graph Systems.}
Probably cut this.
\cite{ammar2018distributed}
\cite{aspire} distributed memory graph processing system which uses a relaxed memory consistency model to reduce communication latency during computation for vertex-centric graph algorithms.
\end{comment}

\paragraph{Distributed Streaming Graph Systems.}
In recent years there have been a variety of distributed graph processing systems designed for graphs which change over time. Kineograph~\cite{kineograph} is a general-purpose framework for incremental graph algorithms which uses snapshots for efficient incremental computation. GraphTau~\cite{graphtau} also uses a graph snapshot method implemented on top of Apache Spark's RDDs for graph analytics in the sliding window model, where edges disappear some fixed number of time steps after their insertion. Kickstarter~\cite{kickstarter} is a runtime technique for incremental monotonic graph algorithms which trims approximate vertex values when edges are deleted to efficiently update the algorithm's result. It is implemented in the distributed graph processing system ASPIRE\cite{aspire}.
CellIQ~\cite{iyer2015celliq} is a distributed graph system optimized for solving the connected components problem on cellular network graphs in the sliding window model. Tegra~\cite{iyer2021tegra} is designed to compute a variety of time-window graph analytics on dynamic graphs. DiStinger~\cite{distinger} is a distributed extension of Stinger~\cite{ediger2012stinger} which is optimized for solving PageRank on sparse graph streams.

==> technical_overview.tex <==
\section{Technical Overview}
We give a brief overview of the techniques that allow \sysname to overcome the CPU, communication, and space bottlenecks.


\paragraph{Overcoming the CPU bottleneck.}
Prior systems using linear sketching algorithms are bottlenecked on CPU cost~\cite{graphzeppelin,l0sketch}.
\sysname overcomes this high CPU cost in two ways: First, via algorithmic improvements that lower the total work required to update the sketches, and second, by distributing this work to worker nodes in the cluster.

\sysname's \sketchname algorithm significantly reduces update cost. Existing algorithms for $\ell_0-$sampling~\cite{graphzeppelin,l0sketch} (the key sampling subroutine for connected components sketching), including the state-of-the-art \cubesketch, have worst-case update time $O(\log^2(\nodesize))$. \sketchname's update time is $O(\log(\nodesize))$, which we show experimentally leads to a $4\times$ speedup over \cubesketch.

\sysname scales well when given more distributed compute power: given 40 distributed workers (with 16 cores each), it can ingest updates $35\times$ faster than with 1 distributed worker (with 16 cores). \sysname's high scalability is a consequence of its linear sketches.  


\paragraph{Overcoming the communication bottleneck.}
For any sequence of graph updates and connectivity queries, the total communication \sysname uses to process the stream and answer each query is at most a $(3 + \epsilon)$ factor larger than the bandwidth required to read in the input stream at the main node. Since any stream-processing system must receive the input stream over a network link at the main node, \sysname is therefore a small constant factor away from the minimum possible communication for any distributed solution to the streaming connected components problem.

\sysname accomplishes this remarkable result by exploiting the data locality properties of its \sketchnames. First, it collects updates into \defn{vertex-based batches}, defined to be a batch of edge updates that share a vertex. This amortizes the communication cost of distributing updates. Each vertex-based batch is processed by a single distributed worker. In Section \label{subsec:pht} we describe how updates are batched using \sysname's \defn{\treename} and in Section \ref{subsec:gzcomp} show how the \treename can process the input stream into batches at 1/3 of sequential RAM bandwidth. Second, \sysname's \defn {batch distribution policy} assigns batches to workers such that queries frequently require no additional communication.
Since its sketches are stored entirely on the main node, if the sketch has processed all pending updates, the query can be computed locally with latency at most twice as high as the best single-machine graph-stream processing systems~\cite{aspen,terrace,graphzeppelin}. If some pending updates have not been processed, the batch distribution policy chooses whether to distribute this work or perform it locally. In Section \ref{subsec:queries}, we describe this batch distribution policy and prove that for any sequence of graph updates and connectivity queries, the total communication required to process the stream and answer each query is at most a $(3 + \epsilon)$ factor larger than the bandwidth required to read in the input stream. %The sequences that produce the worst-case performance are pathological and unlikely to occur in practice; we show experimentally in Section \ref{subsec:queryex} that queries incur negligible communication on realistic inputs. \david{this sounds like a weakener so we need to make it clear that we're talking about getting better performance than the guarantee in almost all real scenarios.}

In certain cases, \sysname can compute queries using no communication at all. \sysname's queries produce a certificate that summarizes connectivity information. \sysname can also be configured to answer further queries more quickly if this certificate is still valid, a technique we call \defn{opportunistic query elision}. It is often possible to locally update the certificate as new graph updates arrive to maintain correctness without repeating the full query algorithm from scratch. Queries answered via opportunistic elision require no network communication whatsoever. \sysname is capable of performing these local updates and monitoring the certificate for correctness. If the input stream introduces updates that violate correctness, the certificate is discarded and the next query is computed from scratch. We show experimentally in Section \ref{subsec:queryex} that this results in a four orders-of-magnitude decrease in query latency for a variety of simulated graph-update and query sequences.


\paragraph{Overcoming the space bottleneck.}
Because \sysname's linear sketches are asymptotically smaller than the graph, they fit on a single node, even when the graph is very large (\ie has many vertices) and is dense. In fact, recent work~\cite{nelson2019optimal} has shown that \sysname's $O(\nodesize \log^3(\nodesize))$ space cost (where $\nodesize$ is the number of vertices in the graph) is asymptotically optimal when computing connected components on a stream with edge insertions and deletions. 

This asymptotic space cost translates to an actual space savings at surprisingly small graph sizes. The most compact lossless representation of a dense graph is an adjacency matrix with a single bit per entry. \sysname uses less space than such an adjacency matrix even when the input graph only has a million vertices, and we demonstrate experimentally that \sysname can still process such graphs at a bandwidth of hundreds of millions of edges per second. \sysname's \sketchnames are 2.3 times smaller than the state-of-the-art \cubesketch used by GraphZeppelin~\cite{graphzeppelin}. 
Specifically, \sysname uses $246(\log^2(\nodesize) - \log(\nodesize))$B of space for a graph on $\nodesize$ vertices.

==> titleauthieee.tex <==
\title{\sysname: Distributed Graph Sketching}

\author{\IEEEauthorblockN{Anonymous Authors}}
